Structured Pruning of a BERT-based Question Answering Model

The recent trend in industry-setting Natural Language Processing (NLP) research has been to operate large %scale pretrained language models like BERT under strict computational limits. While most model compression work has focused on "distilling" a general-purpose language representation using expensive pretraining distillation, less attention has been paid to creating smaller task-specific language representations which, arguably, are more useful in an industry setting. In this paper, we investigate compressing BERT- and RoBERTa-based question answering systems by structured pruning of parameters from the underlying transformer model. We find that an inexpensive combination of task-specific structured pruning and task-specific distillation, without the expense of pretraining distillation, yields highly-performing models across a range of speed/accuracy tradeoff operating points. We start from existing full-size models trained for SQuAD 2.0 or Natural Questions and introduce gates that allow selected parts of transformers to be individually eliminated. Specifically, we investigate (1) structured pruning to reduce the number of parameters in each transformer layer, (2) applicability to both BERT- and RoBERTa-based models, (3) applicability to both SQuAD 2.0 and Natural Questions, and (4) combining structured pruning with distillation. We achieve a near-doubling of inference speed with less than a 0.5 F1-point loss in short answer accuracy on Natural Questions.

==> notation.tex <==
\begin{figure}
\begin{center}
\begin{tabular}{|l|l|r|r|}
\hline
notation &dimension & base & large \\
\hline
$ \nlayers $ & layers & 12 & 24 \\  
$\embeddingdim$ & embeddings & 768 & 1024 \\
$\nheads$ & attention heads & 12 & 16 \\
$\intermediatedim $ & intermediate size & 3072 & 4096 \\
\hline
\end{tabular}
\end{center}
\caption{Notation: important dimensions of a BERT model}
\label{notation}
\end{figure}

The size of a BERT model is characterized by the values in table \ref{notation}.


==> retraining.tex <==


After gates for which $\gamma_i=0$ have been trained by one of the above methods,
, the model is pruned -
corresponding attention heads are removed,
and corresponding slices of the feed forward linear transformations are removed.
The masking vectors themselves are no longer needed.
Then task-specific training of all BERT parameters is continued for an additional epoch.

